On Groups of PL-homeomorphisms of the Real Line

Richard J. Thompson invented his group F in the 60s; it is a group full of surprises: it has a finite presentation with 2 generators and 2 relators, and a derived group that is simple; it admits a peculiar infinite presentation and has a local definition which implies that F is dense in the topological group of all orientation preserving homeomorphisms of the unit interval. In this monograph groups G are studied which depend on three parameters I, A, and P and which generalize the local definition of Thompson's group F thus: G consists of all orientation preserving PL-homeomorphisms of the real line with supports in the interval I, slopes in the multiplicative subgroup P of the positive reals and breaks in a finite subset of the additive P submodule A of R. A first aim of the monograph is to investigate in which form familiar properties of F continue to hold for these groups. Main aims of the monograph are the determination of isomorphisms among the groups G and the study of their automorphism groups. Complete answers are obtained if the group P is not cyclic or if the interval I is the full line.

==> Z.definitions.tex <==
%
\makeatletter
%
%
\DeclareMathOperator{\ab}{ab}
\DeclareMathOperator{\add}{add}
\DeclareMathOperator{\Aff}{Aff}
\DeclareMathOperator{\aff}{aff}
\DeclareMathOperator{\Ann}{Ann}
\DeclareMathOperator{\Att}{Att}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\Autfr}{\mathfrak{Aut}}
%   B
%   C
\DeclareMathOperator{\can}{can}
\DeclareMathOperator{\card}{card}
\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator{\cpl}{cpl}
%   D
%   E
%   F
\DeclareMathOperator{\FP}{FP}
%   G
\DeclareMathOperator{\gp}{gp}
%   H
\DeclareMathOperator{\Homeo}{Homeo}
\DeclareMathOperator{\homeo}{homeo}
%  I
\newcommand{\id}{\mathbbm{1}}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\Inn}{Inn}
\DeclareMathOperator{\Incl}{incl.}
\DeclareMathOperator{\inner}{inner}
\DeclareMathOperator{\Int}{int}
%  L
%   M
\DeclareMathOperator{\md}{md}
%  N
% O
\DeclareMathOperator{\Out}{Out}
\DeclareMathOperator{\Outfr}{\mathfrak{Out}}
\DeclareMathOperator{\Outer}{outer}
%  P
\DeclareMathOperator{\per}{per}
\DeclareMathOperator{\PL}{PL}
\DeclareMathOperator{\PLhomeo}{PL-homeo}
%   R
\DeclareMathOperator{\rk}{rk}
%    S
\DeclareMathOperator{\Sing}{Sing}
\DeclareMathOperator{\St}{St}
\DeclareMathOperator{\supp}{supp}
%  T
\DeclareMathOperator{\Tor}{Tor}
%
%
%% blackboard letters
%%
\DeclareMathOperator{\N}{\mathbb{N}} 
\DeclareMathOperator{\Q}{\mathbb{Q}} 
\DeclareMathOperator{\R}{\mathbb{R}} 
\DeclareMathOperator{\Z}{\mathbb{Z}} 
%
%
%% Calligraphic letters
%
\DeclareMathOperator{\Acal}{\mathcal{A}} 
\DeclareMathOperator{\BB}{\mathcal{B}} 
\DeclareMathOperator{\CC}{\mathcal{C}} 
\DeclareMathOperator{\Fcal}{\mathcal{F}} 
\DeclareMathOperator{\GG}{\mathcal{G}} 
\DeclareMathOperator{\KK}{\mathcal{K}} 
\DeclareMathOperator{\OO}{\mathcal{O}} 
\DeclareMathOperator{\PP}{\mathcal{P}} 
\DeclareMathOperator{\QQ}{\mathcal{Q}} 
\DeclareMathOperator{\RR}{\mathcal{R}} 
\DeclareMathOperator{\Scal}{\mathcal{S}} 
\DeclareMathOperator{\TT}{\mathcal{T}} 
 \DeclareMathOperator{\WW}{\mathcal{W}} 
\DeclareMathOperator{\XX}{\mathcal{X}} 
\DeclareMathOperator{\YY}{\mathcal{Y}} 
\DeclareMathOperator{\ZZ}{\mathcal{Z}} 
%
% eufrak
%
\newcommand{\Afr}{\mathfrak{A}} 
\newcommand{\Bfr}{\mathfrak{B}}
\newcommand{\Ffr}{\mathfrak{F}} 
\newcommand{\pfr}{\mathfrak{p}}
\newcommand{\Sfr}{\mathfrak{S}}
\newcommand{\Tfr}{\mathfrak{T}}

% morphisms
\newcommand{\mono}{\rightarrowtail}
\newcommand{\incl}{\hookrightarrow}
\newcommand{\epi}{\twoheadrightarrow}
\newcommand{\iso}{\stackrel{\sim}{\longrightarrow}}
\newcommand{\isoinv}{\stackrel{\sim}{\longleftarrow}}
%
% useful abbreviations (see LaTeX Companion, page 80)
%
\newcommand{\eg}{e.g., \xspace}
\newcommand{\ie}{i.e., \xspace}
\newcommand{\etc}{etc. \@\xspace}
\newcommand{\cf}{cf. \@\xspace}
%
% command for left conjugation
%
\newcommand{\act}[1]{\,^{#1}}
%
\makeatother
\endinput

==> Z.layout.tex <==
%%
\makeatletter
%
%
%======================
% Theoremlike environments
%======================
%
\theoremheaderfont{\rmfamily\scshape}
%
{\theorembodyfont{\itshape}
\newtheorem{thm}{Theorem}[section]
\newtheorem{theorem}[thm]{Theorem}
\newtheorem{thmNN}{Theorem}
\newtheorem{thmMain}{Theorem}
\newtheorem{prp}[thm]{Proposition}
\newtheorem{proposition}[thm]{Proposition}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{crl}[thm]{Corollary}
\newtheorem{corollary}[thm]{Corollary}
\newtheorem{criterion}{Criterion}
%
\newtheorem{conjecture}[thm]{Conjecture}
\newtheorem{problem}[thm]{Problem}
\newtheorem{supplement}[thm]{Supplement}
\newtheorem{claim}{Claim}
%
% In the preamble, a special way of numerating the results is used.
%
\newtheorem{thmP}{Theorem}[chapter]
\newtheorem{prpP}[thmP]{Proposition}
\newtheorem{crlP}[thmP]{Corollary}
\newtheorem{supplementP}[thmP]{Supplement}

% In the original introduction,
%the results are called Theorem 2.4 etc,.  not  Theorem I2.4 etc.
%
\newtheorem{thmI}{Theorem}[chapter]
\newtheorem{prpI}[thmI]{Proposition}
\newtheorem{crlI}[thmI]{Corollary}
\newtheorem{supplementI}[thmI]{Supplement}
%
% 
% In the notes, 
% another way of numbering the results is used.
%
\newtheorem{thmN}{Theorem}[chapter]
\newtheorem{prpN}[thmN]{Proposition}
\newtheorem{crlN}[thmN]{Corollary}
\newtheorem{supplementN}[thmN]{Supplement}
\newtheorem{characterizationN}[thmN]{Characterization}
}
%
{\theorembodyfont{\upshape}
\newtheorem{convention}[thm]{Convention}
\newtheorem{definition}[thm]{Definition}
\newtheorem{definitions}[thm]{Definitions}
\newtheorem{definitionN}[thmN]{Definition}
\newtheorem{definitionNN}{Definition}
\newtheorem{example}[thm]{Example}
\newtheorem{examples}[thm]{Examples}
\newtheorem{illustration}[thm]{Illustration}
\newtheorem{remark}[thm]{Remark}
\newtheorem{remarks}[thm]{Remarks} 
\newtheorem{note}[thm]{Note}
\newtheorem{rmk}{Remark}
\newtheorem{rmks}{Remarks}
%
\newtheorem{remarkP}[thmP]{Remark}
}
%
%
%----------------
% Numbering of headings
%----------------
\renewcommand{\thechapter}{\Alph{chapter}}
\renewcommand{\thesection}{\arabic{section}}
\renewcommand{\thesubsection}{\thesection.\arabic{subsection}}
\renewcommand{\thesubsubsection}{\thesubsection\alph{subsubsection}}
%
\renewcommand{\thethm}{\Alph{chapter}\thesection.\arabic{thm}}
\renewcommand{\thethmMain}{\thechapter}
\renewcommand{\thethmI}{\thesection.\arabic{thmI}}
\renewcommand{\thethmP}{\arabic{thmP}}
\renewcommand{\thethmNN}{\hspace*{-0.3em}.}
%
\renewcommand{\theequation}{\arabic{section}.\arabic{equation}}
\renewcommand{\thefigure}{\thechapter\arabic{figure}}
%\renewcommand{\theillustration}{\hspace*{-0.3em}.}
%\renewcommand{\theconvention}{\hspace*{-0.3em}.}
\renewcommand{\theclaim}{\hspace*{-0.3em}.}
\renewcommand{\thermk}{\hspace*{-0.3em}.}
\renewcommand{\thermks}{\hspace*{-0.3em}.}
%\renewcommand{\theillu}{\hspace*{-0.3em}.}
%
\renewcommand{\thenote}{\arabic{note}}

%
% Counters            
%--------------
%
\numberwithin{equation}{section}
%
%\@addtoreset{figure}{section}
\@addtoreset{footnote}{chapter}
%\@addtoreset{equation}{section}
%%%
%
% Environment 'proof' 
%----------------------------
%
\newenvironment{proof}%
{\removelastskip%
\vspace{12 pt plus1pt}
\noindent\textit{Proof.}}%
{\hfill $\square$\par \medskip}%

\newenvironment{proof-special}%
{\removelastskip%
\vspace{12 pt plus1pt}
\noindent\textit{Proof.}}%
{\par \medskip}%

%%
%%
% Layout of the page
%------------------------------------
\setlength{\textwidth}{125mm}%
\setlength{\textheight}{190mm}%
\setlength{\oddsidemargin}{1.6cm}%
\setlength{\evensidemargin}{1.6cm}%
\setlength{\headheight}{12pt}%
\setlength{\headsep}{20pt}%
\setlength{\topmargin}{0mm}%
\setlength{\marginparwidth}{\evensidemargin}%
%
\setcounter{totalnumber}{9}
\setcounter{topnumber}{9}
\renewcommand{\topfraction}{0.9}
\renewcommand{\bottomfraction}{0.9}
\renewcommand{\textfraction}{0.1}
\setlength{\floatsep}{6 pt plus 1pt minus 2 pt}
\setlength{\textfloatsep}{6pt plus 1pt minus2pt}%
\setlength{\intextsep}{6pt plus 1pt minus2pt}%
\renewcommand{\floatpagefraction}{0.8}

\renewcommand{\topfraction}{0.95}
\renewcommand{\bottomfraction}{0.7}
\setlength{\floatsep}{6 pt plus 1pt minus 2 pt}
\setlength{\textfloatsep}{6pt plus 1pt minus2pt}%
\setlength{\intextsep}{6pt plus 1pt minus2pt}%
\renewcommand{\floatpagefraction}{1}
%
%-----------------
% Definition of  fonts
%-----------------
\newcommand{\specialfont}{cmss}  
\newcommand{\titlingfontup}{\usefont{T1}{\specialfont}{m}{n}}
\newcommand{\titlingfontit}{\usefont{T1}{\specialfont}{m}{it}}
\newcommand{\headerfont}{\usefont{T1}{\specialfont}{m}{it}}
\newcommand{\pagefont}{\usefont{T1}{\specialfont}{m}{it}}
%
%===================
%
% DEFINITION OF THE VARIOUS STYLES
%
%===================
%
%
%===============
% Defining the chapter styles
%===============
%
\renewcommand{\chapnamefont}{\titlingfontup}
\renewcommand{\chapnumfont}{\chapnamefont}
\renewcommand{\chaptitlefont}{\titlingfontup}
%
%-----------------------------
%  FRONT: chapterstyle
%-----------------------------
%
\makechapterstyle{front}{%
%
\setlength{\beforechapskip}{0pt}
\renewcommand{\printchaptername}{}%
\renewcommand{\printchapternum}{}%
\setlength{\midchapskip}{0pt}%
%
\renewcommand{\printchaptertitle}[1]{%
%\hrule 
\vspace*{0.8\baselineskip}
\centering \titlingfontup \huge  ##1 \par 
\vspace*{0.5\baselineskip}
\hrule
}
%
\setlength{\afterchapskip}{40pt}
}
%
% Code of ToC in the Notes
%
%----------------------------------------
% Modifying Table of Contents
%---------------------------------------
%
\renewcommand\tableofcontents{%
    \if@twocolumn
      \@restonecoltrue\onecolumn
    \else
      \@restonecolfalse
    \fi
    \chapter*{\contentsname
    %----------
        \@mkboth{ \contentsname}{\contentsname}}%
    %----------
    \@starttoc{toc}%
    \if@restonecol\twocolumn\fi
    }
%

%
%
%------------
%  MAIN: chapterstyle
%------------
%
\makechapterstyle{main}{%
%
\renewcommand{\chapnamefont}{\titlingfontup}
\renewcommand{\chapnumfont}{\chapnamefont}
\renewcommand{\chaptitlefont}{\titlingfontup}
%
\setlength{\beforechapskip}{0pt}
\renewcommand{\chapterheadstart}{\vspace*{\beforechapskip} 
%\hrule \vspace*{0.6\baselineskip}
}
%
\renewcommand{\printchaptername}{}%
\renewcommand{\chapternamenum}{}%
\renewcommand{\printchapternum}{}%
\setlength{\midchapskip}{0pt}%
%
\renewcommand{\printchaptertitle}[1]{%
\centering \titlingfontup \huge
\thechapter \quad  ##1 \par%
\vspace*{0.4\baselineskip}\hrule}
\setlength{\afterchapskip}{40pt}
}
%
%---------------
% chapterstyle for bibliography
%--------------

\renewenvironment{thebibliography}[1]{%
%
\chapter*{\bibname}%
      \@mkboth{\bibname}{\bibname}%
      \list{\@biblabel{\@arabic\c@enumiv}}%
           {\settowidth\labelwidth{\@biblabel{#1}}%
            \leftmargin\labelwidth
            \advance\leftmargin\labelsep
            \@openbib@code
            \usecounter{enumiv}%
            \let\p@enumiv\@empty
            \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      \sloppy
      \clubpenalty4000
      \@clubpenalty \clubpenalty
      \widowpenalty4000%
      \sfcode`\.\@m}
     {\def\@noitemerr
       {\@latex@warning{Empty `thebibliography' environment}}%
      \endlist}
%


%------------
% chapterstyle for Notes
%------------
%
\makechapterstyle{back}{%
%
\setlength{\beforechapskip}{0pt}
\renewcommand{\printchaptername}{}%
\renewcommand{\printchapternum}{}%
\setlength{\midchapskip}{0pt}%
%
\renewcommand{\printchaptertitle}[1]{%
\hrule 
\vspace*{0.8\baselineskip}
\centering \titlingfontup \huge  ##1 \par 
\vspace*{0.4\baselineskip}
\hrule}
%
\setlength{\afterchapskip}{50pt}
}
%

%---------------
% pagestyles for Front Matter
%---------------
%
%\makepagestyle{front}%
%\renewcommand{\chaptermark}[1]{\markboth {#1}{}}%
%\renewcommand{\sectionmark}[1]{\markright {#1}}%
%
%
\makepagestyle{frontP}
\makeheadrule{frontP}{\textwidth}{\normalrulethickness}
%
\makeoddhead{frontP}%
{\headerfont \footnotesize Preface}{}%
{\pagefont \footnotesize \thepage}%
%
\makeevenhead{frontP}%
{\pagefont\footnotesize\thepage}{}%
{\headerfont\footnotesize Preface}%
%
%
\makepagestyle{frontToC}
\makeheadrule{frontToC}{\textwidth}{\normalrulethickness}
%
\makeoddhead{frontToC}%
{\headerfont \footnotesize Table of Contents}{}%
{\pagefont \footnotesize \thepage}%
%
\makeevenhead{frontToC}%
{\pagefont\footnotesize\thepage}{}%
{\headerfont\footnotesize Table of Contents}%

%
%\makepagestyle{main-plain}
%\makeevenfoot{main-plain}{}{\pagefont  \footnotesize \thepage}{}
%\makeoddfoot{main-plain}{}{\pagefont  \footnotesize \thepage}{}
%%
%%
%\makeevenfoot{main-plain}{}{\pagefont  \footnotesize \thepage}{}
%\makeoddfoot{main-plain}{}{\pagefont  \footnotesize \thepage}{}



%---------------
% pagestyle for Main Matter
%---------------
%
\makepagestyle{main}%
\renewcommand{\chaptermark}[1]{\markboth {#1}{}}%
\renewcommand{\sectionmark}[1]{\markright {#1}}%
%
%
\makeheadrule{main}{\textwidth}{\normalrulethickness}
%
\makeoddhead{main}%
{\headerfont \footnotesize \thesection\quad \rightmark}{}%
{\pagefont \footnotesize \thepage}%
%
\makeevenhead{main}%
{\pagefont\footnotesize\thepage}{}%
{\headerfont\footnotesize \thechapter \quad \leftmark}%
%
\makepagestyle{main-plain}
\makeevenfoot{main-plain}{}{\pagefont  \footnotesize \thepage}{}
\makeoddfoot{main-plain}{}{\pagefont  \footnotesize \thepage}{}
%
%
\makeevenfoot{main-plain}{}{\pagefont  \footnotesize \thepage}{}
\makeoddfoot{main-plain}{}{\pagefont  \footnotesize \thepage}{}

%
%

%---------------------
% pagestyles for Back Matter
%--------------------
%
\makepagestyle{backB}
%
\makeheadrule{backB}{\textwidth}{\normalrulethickness}%
\makeoddhead{backB}%
{\headerfont \footnotesize Bibliography}{}{\pagefont \footnotesize \thepage}%
%
\makeevenhead{backB}%
{\pagefont\footnotesize\thepage}{}{\headerfont\footnotesize Bibliography}%

\makepagestyle{backSI}
%
\makeheadrule{backSI}{\textwidth}{\normalrulethickness}%
\makeoddhead{backSI}%
{\headerfont \footnotesize Subject Index}{}{\pagefont \footnotesize \thepage}%
%
\makeevenhead{backSI}%
{\pagefont\footnotesize\thepage}{}{\headerfont\footnotesize Subject Index}%

%===============
%  commands for sections
%================
%
\setsecheadstyle{%
\titlingfontup\fontsize{14}{16pt}\selectfont \raggedright}
%
\setsubsecheadstyle{%
\titlingfontup\fontsize{12}{14pt}\selectfont \raggedright}
%
\setsubsubsecheadstyle{
\titlingfontit   \fontsize{10}{12pt}\selectfont \raggedright}
%
\setparaheadstyle{%
\titlingfontit  \fontsize{10}{12.0pt}\selectfont \raggedright}

%
%----------------
%%
\makeatother
\endinput

==> chaptB.9.5.FigureB1.tex <==
%
% First part
%
\begin{minipage}{12 cm}
%
% function f1
%
\psfrag{1}{\hspace*{-1.7mm}   \footnotesize 0}
\psfrag{2}{\hspace*{-1.6mm}  \footnotesize $\tfrac{1}{3}$}
\psfrag{3}{\hspace*{-1.8mm} \footnotesize $\tfrac{1}{2}$}
\psfrag{4}{\hspace*{-0.5mm}\footnotesize  $\tfrac{2}{3}$}
\psfrag{5}{\hspace*{-1.1mm}  \footnotesize  1}
%
\psfrag{11}{\hspace*{-0.7mm}  \footnotesize  $0$}
\psfrag{12}{\hspace*{-0,9 mm}  \footnotesize$\tfrac{1}{6}$}
\psfrag{13}{\hspace*{-1.0mm}  \footnotesize $\tfrac{1}{3}$}
\psfrag{14}{\hspace*{-0.9mm}  \footnotesize$\tfrac{2}{3}$}
\psfrag{15}{\hspace*{-0.7mm}  \footnotesize $1$}
%
\psfrag{21}{\hspace*{-1.7mm} \footnotesize $\tfrac{1}{2}$}
\psfrag{22}{  \hspace*{-1.0mm}\footnotesize  1}
\psfrag{23}{\hspace*{-1mm} \footnotesize 2}
\psfrag{24}{\hspace*{-1.0mm} \footnotesize 1}
%
% function f2
%
\psfrag{31}{\hspace*{-0.6mm}    \footnotesize $0$}
\psfrag{32}{\hspace*{-1.0mm}   \footnotesize $\tfrac{1}{3}$}
\psfrag{33}{\hspace*{-0.9mm}  \footnotesize $\tfrac{2}{3}$}
\psfrag{34}{\hspace*{-0.9mm} \footnotesize  $\tfrac{5}{6}$}
\psfrag{35}{\hspace*{-0.6mm}   \footnotesize  $1$}
%
%
\psfrag{41}{\hspace*{-0.2mm}  \footnotesize  $0$}
\psfrag{42}{\hspace*{-0.6mm}  \footnotesize$\tfrac{1}{6}$}
\psfrag{43}{\hspace*{-0.6mm}  \footnotesize $\tfrac{1}{3}$}
\psfrag{44}{\hspace*{-0.6mm}  \footnotesize$\tfrac{2}{3}$}
\psfrag{45}{\hspace*{-0.4mm}  \footnotesize $1$}
%
\psfrag{51}{\hspace*{-1.7mm}  \footnotesize $\tfrac{1}{2}$}
\psfrag{52}{  \hspace*{-2.5mm} \footnotesize  $\tfrac{1}{2}$}
\psfrag{53}{\hspace*{-1mm}  \footnotesize 2}
\psfrag{54}{\hspace*{-1.0mm}  \footnotesize 2}
%
% function f3
%
\psfrag{61}{\hspace*{-0.5mm}   \footnotesize $0$}
\psfrag{62}{\hspace*{-0.7mm}  \footnotesize $\tfrac{1}{6}$}
\psfrag{63}{\hspace*{-0.9mm} \footnotesize $\tfrac{1}{3}$}
\psfrag{64}{\hspace*{-0.6 mm}\footnotesize   $\tfrac{5}{12}$}
\psfrag{65}{\hspace*{-1.0mm}  \footnotesize $\tfrac{1}{2}$}
\psfrag{66}{\hspace*{-0.6mm}  \footnotesize  $1$}
%
%
\psfrag{71}{\hspace*{-0.4mm} \footnotesize  $0$}
\psfrag{72}{\hspace*{-1.2mm} \footnotesize $\tfrac{1}{12}$}
\psfrag{73}{\hspace*{-0.4mm} \footnotesize $\tfrac{1}{6}$}
\psfrag{74}{\hspace*{-0.7mm} \footnotesize $ \tfrac{1}{3}$}
\psfrag{75}{\hspace*{-0.7mm}  \footnotesize $\tfrac{1}{2}$}
\psfrag{76}{\hspace*{-0.4mm} \footnotesize$1$}
%
\psfrag{81}{\hspace*{-0.8mm} \footnotesize $\tfrac{1}{2}$}
\psfrag{82}{  \hspace*{-1.3mm}\footnotesize  $\tfrac{1}{2}$}
\psfrag{83}{\hspace*{-0.5mm} \footnotesize 2}
\psfrag{84}{\hspace*{-0.5mm} \footnotesize 2}
\psfrag{85}{  \hspace*{-1.0mm}\footnotesize 1}
%
\psfrag{la1}{\hspace{-1mm}$f_1$}
\psfrag{la2}{\hspace{-2.5mm} $f_2$}
\psfrag{la3}{\hspace{-2mm}$f_3$}
%
\begin{gather*}
\includegraphics[width= 5.5cm]{BiSt.chaptB.fig2.eps}
\hspace*{6mm}
\includegraphics[width= 5.5cm]{BiSt.chaptB.fig3.eps}
\\
\includegraphics[width= 5.5cm]{BiSt.chaptB.fig4.eps}
\end{gather*}
%
\end{minipage}
%
% second part
\begin{minipage}{12cm}
%
% function f1
%
\psfrag{1}{\hspace*{-1.4mm}   \small 0}
\psfrag{2}{\hspace*{-2.3mm}  \small $\tfrac{1}{15}$}
\psfrag{3}{\hspace*{-2.4mm} \small $\tfrac{2}{15}$}
\psfrag{4}{\hspace*{-1.2mm}\small  $\tfrac{3}{15}$}
\psfrag{5}{\hspace*{-2.5mm}  \small  $\tfrac{4}{15}$}
\psfrag{6}{\hspace*{-1.6mm}  \small  $\tfrac{1}{3}$}
\psfrag{7}{\hspace*{-1.7mm}  \small  $\tfrac{2}{3}$}
\psfrag{8}{\hspace*{-1.4mm}  \small  1}
%
\psfrag{11}{\hspace*{-0.7mm}  \small  $0$}
\psfrag{12}{\hspace*{-0.9mm}  \small$\tfrac{1}{7}$}
\psfrag{13}{\hspace*{-0.9mm}  \small $\tfrac{2}{7}$}
\psfrag{14}{\hspace*{-0.9mm}  \small$\tfrac{3}{7}$}
\psfrag{15}{\hspace*{-1.0mm}   \small $\tfrac{4}{7}$}
\psfrag{16}{\hspace*{-0.8mm}   \small$\tfrac{5}{7}$}
\psfrag{17}{\hspace*{-1.0mm}   \small $\tfrac{6}{7}$}
\psfrag{18}{\hspace*{-0.5mm}   \small $1$}
%
\psfrag{21}{\hspace*{-1.8mm}  \small $\tfrac{15}{7}$}
\psfrag{22}{\hspace*{-2.0mm} \small $\tfrac{15}{7}$}
\psfrag{23}{\hspace*{-1.8mm}   \small $\tfrac{15}{7}$}
\psfrag{24}{\hspace*{-2.0mm}  \small $\tfrac{15}{7}$}
\psfrag{25}{\hspace*{-1.0mm}  \small $\tfrac{15}{7}$}
\psfrag{26}{\hspace*{1.3mm}  \small $\tfrac{3}{7}$}
\psfrag{27}{\hspace*{1.5mm}  \small $\tfrac{3}{7}$}
%
\psfrag{laH357}{\hspace{-8mm}\small $h(3,5;7)$}
%
\begin{equation*}
\includegraphics[width= 10.5cm]{BiSt.chaptB.fig5.eps}
\end{equation*}
%
\end{minipage}
%
% Third part
%
\begin{minipage}{12 cm}
%
% function t(1;3,5)
%
\psfrag{1}{\hspace*{-1.7mm}   \small 0}
\psfrag{2}{\hspace*{-2.5mm}  \small $\tfrac{1}{15}$}
\psfrag{3}{\hspace*{-2.5mm} \small $\tfrac{2}{15}$}
\psfrag{4}{\hspace*{-1.0mm}\small  $\tfrac{3}{15}$}
\psfrag{5}{\hspace*{-1.9mm}  \small  $\tfrac{4}{15}$}
\psfrag{6}{\hspace*{-1.8mm}  \small  $\tfrac{1}{3}$}
\psfrag{7}{\hspace*{-1.7mm}  \small  $\tfrac{2}{3}$}
\psfrag{8}{\hspace*{-1.5mm}  \small  1}
%
\psfrag{11}{\hspace*{-0.7mm}  \small  $0$}
\psfrag{12}{\hspace*{-1.7mm}  \small$\tfrac{1}{15}$}
\psfrag{13}{\hspace*{-1.7mm}  \small $\tfrac{2}{15}$}
\psfrag{14}{\hspace*{-1.0mm}  \small$\tfrac{1}{5}$}
\psfrag{15}{\hspace*{-1.0mm}   \small $\tfrac{2}{5}$}
\psfrag{16}{\hspace*{-0.8mm}   \small$\tfrac{3}{5}$}
\psfrag{17}{\hspace*{-1.0mm}   \small $\tfrac{4}{5}$}
\psfrag{18}{\hspace*{-0.7mm}   \small $1$}
%
\psfrag{21}{\hspace*{-0.8mm}  \small 1}
\psfrag{22}{\hspace*{-0.8mm} \small 1}
\psfrag{23}{\hspace*{-1mm}   \small 1}
\psfrag{24}{\hspace*{-2.0mm}  \small 3}
\psfrag{25}{\hspace*{-2.0mm}  \small 3}
\psfrag{26}{\hspace*{2.0mm}  \small $\tfrac{3}{5}$}
\psfrag{27}{\hspace*{-1.0mm}  \small $\tfrac{3}{5}$}
%
% function t(2:3.5)
%
\psfrag{31}{\hspace*{-1.0mm}   \small 0}
\psfrag{32}{\hspace*{-1.5mm}  \small $\tfrac{1}{30}$}
\psfrag{33}{\hspace*{-2.7mm} \small }
\psfrag{34}{\hspace*{-0.5mm}\small  $\tfrac{1}{10}$}
\psfrag{35}{\hspace*{-1.7mm}  \small }
\psfrag{36}{\hspace*{-1.0mm}  \small  $\tfrac{1}{6}$}
\psfrag{37}{\hspace*{-0.8mm}  \small  $\tfrac{1}{3}$}
\psfrag{38}{\hspace*{-1.0mm}  \small  $\tfrac{1}{2}$}
\psfrag{39}{\hspace*{-0.5mm}  \small  1}

%
\psfrag{41}{\hspace*{-0.7mm}  \small  $0$}
\psfrag{42}{\hspace*{-1.5mm}  \small$\tfrac{1}{30}$}
\psfrag{43}{\hspace*{-1.6mm}  \small }
\psfrag{44}{\hspace*{-1.3mm}  \small$\tfrac{1}{10}$}
\psfrag{45}{\hspace*{-1.2mm}   \small $\tfrac{2}{10}$}
\psfrag{46}{\hspace*{-1.2mm}   \small$\tfrac{3}{10}$}
\psfrag{47}{\hspace*{-1.3mm}   \small $\tfrac{4}{10}$}
\psfrag{48}{\hspace*{-0.8mm}  \small  $\tfrac{1}{2}$}
\psfrag{49}{\hspace*{-0.3mm}  \small  1}
%%
\psfrag{51}{\hspace*{-0.3mm}  \small 1}
\psfrag{52}{\hspace*{-0.3mm} \small 1}
\psfrag{53}{\hspace*{-0.3mm}   \small 1}
\psfrag{54}{\hspace*{-0.7mm}  \small 3}
\psfrag{55}{\hspace*{-1.0mm}  \small 3}
\psfrag{56}{\hspace*{-1.0mm}  \small $\tfrac{3}{5}$}
\psfrag{57}{\hspace*{-1.0mm}  \small $\tfrac{3}{5}$}
\psfrag{58}{\hspace*{-1.0mm}  \small 1}
%%
%%%
\psfrag{laT135}{\small\hspace{-7mm}$t(1;3,5)$}
\psfrag{laT235}{\small \hspace{-7.5mm} $t(2;3,5)$}
%
\begin{gather*}
\includegraphics[width= 10.5cm]{BiSt.chaptB.fig6.eps}
\\
\includegraphics[width= 10.5cm]{BiSt.chaptB.fig7.eps}
%
\end{gather*}
%
\end{minipage}
%
%% Fourth part
%
\begin{minipage}{12cm}
%
% function g(2;3)
%
\psfrag{1}{\hspace*{-1.5mm}   \small 0}
\psfrag{2}{\hspace*{-1.5mm}  \small $\tfrac{1}{4}$}
\psfrag{3}{\hspace*{-1.6mm} \small $\tfrac{1}{2}$}
\psfrag{4}{\hspace*{-1.2mm}  \small  1}
%
\psfrag{11}{\hspace*{-0.7mm}  \small  $0$}
\psfrag{12}{\hspace*{-0.9mm}  \small$\tfrac{1}{3}$}
\psfrag{13}{\hspace*{-0.9mm}  \small $\tfrac{2}{3}$}
\psfrag{14}{\hspace*{-0.6mm}   \small $1$}
%
\psfrag{21}{\hspace*{-1.7mm}  \small $\tfrac{4}{3}$}
\psfrag{22}{\hspace*{-1.5mm} \small $\tfrac{4}{3}$}
\psfrag{23}{\hspace*{-0.0mm}   \small $\tfrac{2}{3}$}
%
% function g(2;5)
%
\psfrag{31}{\hspace*{-0.7mm}   \small 0}
\psfrag{32}{\hspace*{-1.6mm}  \small $\tfrac{1}{16}$}
\psfrag{33}{\hspace*{-0.8mm} \small $\tfrac{1}{8}$}
\psfrag{34}{\hspace*{0.35mm}\small  $\tfrac{1}{4}$}
\psfrag{35}{\hspace*{-0.7mm}  \small  $\tfrac{1}{2}$}
\psfrag{36}{\hspace*{-0.7mm}  \small  1}
%
\psfrag{41}{\hspace*{-0.2mm}  \small  $0$}
\psfrag{42}{\hspace*{-0.6mm}  \small$\tfrac{1}{5}$}
\psfrag{43}{\hspace*{-0.7mm}  \small $\tfrac{2}{5}$}
\psfrag{44}{\hspace*{-0.8mm}  \small$\tfrac{3}{5}$}
\psfrag{45}{\hspace*{-0.6mm}   \small $\tfrac{4}{5}$}
\psfrag{46}{\hspace*{-0.4mm}   \small $1$}
%
\psfrag{51}{\hspace*{-1.5mm}  \small $\tfrac{16}{5}$}
\psfrag{52}{\hspace*{-1.7mm} \small $\tfrac{16}{5}$}
\psfrag{53}{\hspace*{-0.8mm}   \small $\tfrac{8}{5}$}
\psfrag{54}{\hspace*{-0.0mm}  \small $\tfrac{4}{5}$}
\psfrag{55}{\hspace*{1.5mm}  \small $\tfrac{2}{5}$}
%
% function g(3;5)
%
\psfrag{61}{\hspace*{-0.8mm}   \small 0}
\psfrag{62}{\hspace*{-2.7mm}  \small }
\psfrag{63}{\hspace*{-2.7mm} \small }
\psfrag{64}{\hspace*{-0.4mm}\small  $\tfrac{1}{27}$}
\psfrag{65}{\hspace*{-1.7mm}  \small  }
\psfrag{66}{\hspace*{-0.9mm}  \small  $\tfrac{1}{9}$}
\psfrag{67}{\hspace*{-1.2mm}  \small  $\tfrac{2}{9}$}
\psfrag{68}{\hspace*{-1.0mm}  \small  $\tfrac{1}{3}$}
\psfrag{69}{\hspace*{-1.0mm}  \small  $\tfrac{2}{3}$}
\psfrag{70}{\hspace*{-0.6mm}  \small  1}
%
%%
\psfrag{71}{\hspace*{-0.7mm}  \small  $0$}
\psfrag{72}{\hspace*{-1.2mm}  \small$\tfrac{1}{25}$}
\psfrag{73}{\hspace*{-1.6mm}  \small }
\psfrag{74}{\hspace*{-1.6mm}  \small}
\psfrag{75}{\hspace*{-1.6mm}   \small }
\psfrag{76}{\hspace*{-0.4mm}   \small$\tfrac{1}{5}$}
\psfrag{77}{\hspace*{-0.6mm}   \small $\tfrac{2}{5}$}
\psfrag{78}{\hspace*{-0.6mm}   \small $\tfrac{3}{5}$}
\psfrag{79}{\hspace*{-0.6mm}   \small $\tfrac{4}{5}$}
\psfrag{80}{\hspace*{-0.5mm}   \small $1$}
%%
\psfrag{81}{\hspace*{-2.2mm}  \small }
\psfrag{82}{\hspace*{-2.5mm}  \small }
\psfrag{83}{\hspace*{-2mm}   \small }
\psfrag{84}{\hspace*{-2.0mm}  \small }
\psfrag{85}{\hspace*{-1.5mm}  \small $\tfrac{27}{25}$}
\psfrag{86}{\hspace*{-1.05mm}  \small $\tfrac{9}{5}$}
\psfrag{87}{\hspace*{-1.7mm}  \small $\tfrac{9}{5}$}
\psfrag{88}{\hspace*{2.0mm}  \small $\tfrac{3}{5}$}
\psfrag{89}{  \hspace*{-1.2mm}\small $\tfrac{3}{5}$}
%%
\psfrag{la2G3}{\hspace{-7mm} $g(2,3)$}
\psfrag{la2G5}{\hspace{-7mm} $g(2,5)$}
\psfrag{la3G5}{\hspace{-7mm} $g(3,5)$}
%
\begin{center}
%\hspace*{6mm}
\includegraphics[width= 5.2cm]{BiSt.chaptB.fig8.eps}
%
\hspace*{8mm}
\includegraphics[width= 5.2cm]{BiSt.chaptB.fig9.eps}\par
%
\vspace*{2mm} \hspace*{5mm}
\includegraphics[width= 10.6cm]{BiSt.chaptB.fig10.eps}
\end{center}
%
\end{minipage}
%
 




